Continual Optimization with Symmetry Teleportation for Multi-Task Learning

Multi-task learning (MTL) is a widely explored paradigm that enables the simultaneous learning of multiple tasks using a single model. Despite numerous solutions, the key issues of optimization conflict and task imbalance remain under-addressed, limiting performance. Unlike existing optimization-based approaches that typically reweight task losses or gradients to mitigate conflicts or promote progress, we propose a novel approach based on Continual Optimization with Symmetry Teleportation (COST). During MTL optimization, when an optimization conflict arises, we seek an alternative loss-equivalent point on the loss landscape to reduce conflict. Specifically, we utilize a low-rank adapter (LoRA) to facilitate this practical teleportation by designing convergent, loss-invariant objectives. Additionally, we introduce a historical trajectory reuse strategy to continually leverage the benefits of advanced optimizers. Extensive experiments on multiple mainstream datasets demonstrate the effectiveness of our approach. COST is a plug-and-play solution that enhances a wide range of existing MTL methods. When integrated with state-of-the-art methods, COST achieves superior performance.

==> tables/ablation_app.tex <==
\begin{table}[htbp]
\centering
\caption{Ablation study of CAGrad + \texttt{COST} on CityScapes (2 tasks).}
\label{app_table:ablation}
\begin{tabular}{ccc|c}
\toprule
$\mathcal{L}_t$ & $\mathcal{L}_s$ & HTR  & \textbf{$\Delta$m\% $\downarrow$} \\ \midrule
                   &                     &                     & 11.58 \\
\checkmark         &                     &                     & - \\
-                  & \checkmark          &                     & -  \\
\checkmark         & \checkmark          &            &  9.96  \\ \midrule
\checkmark         & \checkmark          & \checkmark          & \textbf{8.37} \\ \bottomrule
\end{tabular}
\end{table}
